Training with Ciphers to Enhance In-Context Terminology Learning For Translation from Rare Languages

Fine-tuning LLMs with in-context examples (IC-Train) lets translation models adapt to new parallel data at deployment, but it is unclear whether they actually learn the translations of rare terms from those examples. We formalize this capability as in-context term learning (ICTL). We show that standard IC-Train develops this capability only weakly, and propose RareCipherFT, which strengthens it without any lexical resources. RareCipherFT pairs each training target with in-context examples that share a rare term with it. It then replaces that term with a character-shuffled cipher in both the context and the reference, so the term can only be recovered by copying from context. The ciphered fraction of training data is annealed to preserve translation quality. Across seven translation directions between English and Tamil, Assamese, Mizo, Nepali and Hausa, and four models from 1B to 7B parameters, RareCipherFT raises term recall over standard IC-Train by 5-15 absolute points without lowering COMET. Probes using synonyms, nonce words and controls for shared surface context show that these gains come from linking source terms to their in-context translations rather than from shortcuts.

==> illustration.tex <==
\begin{figure}[hbt]
\centering
\small
\begin{tikzpicture}[
    token/.style={
        draw,
        rounded corners=2pt,
        minimum width=0.65cm,
        minimum height=0.45cm,
        inner sep=1pt
    },
    cipher/.style={
        token,
        fill=blue!15,
        font=\bfseries
    },
    arr/.style={->, thick}
]

%-----------------------------
% Top row: target sequence
%-----------------------------
\node at (-0.9,0) {$\cdots$};
\node[token] (w1) at (0,0) {$w_{i-2}$};
\node[token] (w2) at (1.0,0) {$w_{i-1}$};
\node[token] (w3) at (2.0,0) {$w_{i}$};

\node[token,fill=green!15] (w4) at (3.0,0) {$w_{i+1}$};
\node[token,fill=green!15] (w5) at (4.0,0) {$w_{i+2}$};

\node[token] (w6) at (5.0,0) {$w_{i+3}$};
\node at (5.9,0) {$\cdots$};

%-----------------------------
% Bottom row: labels
%-----------------------------
\node at (-0.9,-1.1) {$\cdots$};
\node[token] (l1) at (0,-1.1) {$w_{i-1}$};
\node[token] (l2) at (1.0,-1.1) {$w_{i}$};

\node[cipher] (ck) at (2.0,-1.1) {$c$};

\node[token] (l4) at (3.0,-1.1) {$w_{i+2}$};
\node[token] (l5) at (4.0,-1.1) {$w_{i+3}$};
\node[token] (l6) at (5.0,-1.1) {$w_{i+4}$};
\node at (5.9,-1.1) {$\cdots$};

%-----------------------------
% Arrows
%-----------------------------
\draw[arr] (w1) -- (l1);
\draw[arr] (w2) -- (l2);
\draw[arr] (w3) -- (ck);
\draw[arr] (w4) -- (l4);
\draw[arr] (w5) -- (l5);
\draw[arr] (w6) -- (l6);

%-----------------------------
% Span brace
%-----------------------------
\draw[
decorate,
decoration={brace,amplitude=3pt}
]
(2.7,0.42) -- (4.3,0.42)
node[midway,above=4pt,font=\scriptsize]
{shared word span};

%-----------------------------
% Annotation
%-----------------------------
\draw[->,thick,blue]
(2.0,-1.7) -- (ck.south);

\node[
align=center,
font=\scriptsize,
text width=3.0cm
]
at (2.0,-2)
{Label before span start is\\replaced by cipher token};

\end{tikzpicture}

\caption{\label{fig:spl_label_seq}
Modified next-token supervision for cipher-token training. The top row shows the original target sequence, while the bottom row shows the labels used for the next-token prediction objective. The target sequence (top) remains unchanged. If a selected matching span begins at token $w_{i+1}$, the next-token label for the preceding position ($w_i$) is replaced with the corresponding cipher token $c$, while all other labels remain unchanged.
}

\label{fig:cipher_label}
\end{figure}
